SMT-Based Dynamic Multi-Robot Task Allocation

Multi-Robot Task Allocation (MRTA) is a problem that arises in many application domains including package delivery, warehouse robotics, and healthcare. In this work, we consider the problem of MRTA for a dynamic stream of tasks with task deadlines and capacitated agents (capacity for more than one simultaneous task). Previous work commonly focuses on the static case, uses specialized algorithms for restrictive task specifications, or lacks guarantees. We propose an approach to Dynamic MRTA for capacitated robots that is based on Satisfiability Modulo Theories (SMT) solving and addresses these concerns. We show our approach is both sound and complete, and that the SMT encoding is general, enabling extension to a broader class of task specifications. We show how to leverage the incremental solving capabilities of SMT solvers, keeping learned information when allocating new tasks arriving online, and to solve non-incrementally, which we provide runtime comparisons of. Additionally, we provide an algorithm to start with a smaller but potentially incomplete encoding that can iteratively be adjusted to the complete encoding. We evaluate our method on a parameterized set of benchmarks encoding multi-robot delivery created from a graph abstraction of a hospital-like environment. The effectiveness of our approach is demonstrated using a range of encodings, including quantifier-free theories of uninterpreted functions and linear or bitvector arithmetic across multiple solvers.

==> sections/alternative_encodings.tex <==
\section{Alternative Encodings}

This section should be used to describe the other encoding (SAT, SMT, various different constraints tried) if there is space. Likely we will need to move this to some sort of arxiv appendix.

==> sections/discussion.tex <==
\section{Discussion}

Here we want to provide more discussion on the results and also a bit more information about how we could extend this encoding to include other constraints which makes it more of a general framework than many heuristic approaches.

==> sections/old_encoding_file.tex <==
\subsection{SMT Encoding}

Fig. \ref{fig:encoding} includes the types of constraints that are used in our encoding. We include all for the initial solve and then some are iteratively removed and added for additional solves as explained in Algorithm \ref{alg:overall}. Assume $t_{max}$ is set large enough to be greater than the maximum deadline of any task to appear plus maximum travel time between any two points.

For readability, we also make the following defines:
\begin{align}
    \pickup \ = & \ ITE((\dpid \ \& \ 1 = mod(\numagents, 2)) \wedge (\dpid > \numagents), 1, 0) \label{eq:pick}\\
    \dropoff \ = & \ ITE((\dpid \ \& \ 1 = abs(mod(\numagents, 2) - 1)) \wedge (\dpid > \numagents), 1, 0) \label{eq:drop}\\
    \droplater \ = & \ ( {\bigvee \nolimits_{\dpvar' = \dpvar + 1}^{D - 1} \dpid[\agent][\dpvar'] = 2\task + \numagents + 1} ) \vee False \label{eq:droplater} \\
    \agentstarts \ = & \ \bigvee \nolimits_{\dpvar = 1}^{\numdp - 1} \dpid = 2\task + \numagents \label{ eq:agentstarts} \\
    \validid \ = & \ (\numagents \leq \dpid) \wedge (\dpid < 2\numtasks + \numagents) \label{eq:valid}
\end{align}

\iffalse
\begin{align}
    \conjunctionoveragents & \dptuple[\agent][0] = (\agent, \initload, \inittime) \label{enc:init_dp} \tag{E.\theencodingcounter}
    \\
    %\conjunctionoveragents (\load_{D-1}^n = 0) \\
    \conjunctionoveragents &
    \conjunctionoveractionpoints (\dpload \geq 0) \wedge (\dpload \leq \capacity) \label{enc:bound_load} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionoveractionpoints \dptime \geq \prevdptime + Dist(Room(\dpid), Room(\prevdpid)) \label{enc:valid_travel_time} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \bigwedge \limits_{\dpvar = 1}^{\numdp - 2} (\dpid = \agent) \Rightarrow (\nextdpid = \agent) \label{enc:stay_home} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionoveractionpoints \conjunctionovertasks (\dpid = 2\task + \numagents) \Rightarrow ((\taskstarttime = \dptime) \wedge (\taskagent = \agent) \wedge \droplater) \label{enc:started_task} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionoveractionpoints \conjunctionovertasks (\dpid = 2\task + 1 + \numagents) \Rightarrow ((\taskendtime = \dptime) \wedge (\taskagent = \agent)) \label{enc:ended_task} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionovertasks (\taskagent = \agent) \Rightarrow \agentstarts \label{enc:assigned_agent} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionoveractionpoints (\validid) \Rightarrow \dptime \geq Dist(Room(\dpid), Room(\prevdpid)) + \taskarrivaltime \label{enc:leave_after_arrival} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\ 
    \conjunctionovertasks & (\taskagent \geq 0) \wedge (\taskagent < \numagents) \label{enc:valid_agent} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionovertasks & (\taskstarttime \geq 0) \wedge (\taskendtime \leq \taskdeadline) \label{enc:valid_start_and_end_time} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionovertasks & \taskendtime \geq \taskstarttime + Dist(Room(2\task + \numagents), Room(2\task + \numagents + 1)) \label{enc:enough_travel_time} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoverlocations[\location_1] & \conjunctionoverlocations[\location_2] Dist(\location_1, \location_2) = \locationstopathmapping(\location_1, \location_2)[1] \label{enc:dist_UF} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & Room(\agent) = n_s \label{enc:room_UF_agents} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionovertasks & Room(2\task + \numagents) = m_{s_i} \label{enc:room_UF_task_starts} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionovertasks & Room(2\task + \numagents + 1) = m_{s_f} \label{enc:room_UF_task_ends} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \conjunctionoveractionpoints \dpload = \prevdpload + \pickup - \dropoff \label{enc:load_tracking} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \\
    \conjunctionoveragents & \bigwedge \limits_{\dpvar = 1}^{\numdp - 1} \neg(\dpid = \agent) \Rightarrow (\neg(\prevdpid = \dpid) \wedge (\validid)) \label{enc:at_home_or_doing_task} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
\end{align}
\fi

\ref{enc:init_and_allowed_dp} initializes the action tuples, \ref{enc:stay_home} - \ref{enc:doing_tasks} relate action tuple pairs, \ref{enc:room_UF_agents_and_dist_UF} restrict the uninterpreted functions, \ref{enc:bound_load_bound_id_go_home} - \ref{enc:at_home_or_doing_task_with_id} bound action point values, \ref{enc:room_UF_task_rooms} restrict the task uninterpreted functions, \ref{enc:started_task} - \ref{enc:assigned_agent} related action and task tuples, and \ref{enc:valid_agent_and_times} restrict task tuples.


\begin{figure}[h]
    \centering
    % Updated encoding to match implementation
    \begin{align}
        \conjunctionoveragents & \dptuple[\agent][0] = (\agent, \initload, \inittime) \conjunctionoverdplist \assumelist[\dpindex] \Rightarrow (\dpid[\agent][\dplist[\dpindex]] = \agent) \label{enc:init_and_allowed_dp} 
        %\label{enc:e1}
        \tag{E.\theencodingcounter}
        \\
    %Relating action tuples:
        \iffalse
        \conjunctionoveragents & \conjunctionoveractionpoints \dptime \geq \prevdptime + Dist(Room(\dpid), Room(\prevdpid)) \label{enc:valid_travel_time}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \fi
        \conjunctionoveragents & \bigwedge \nolimits_{\dpvar = 1}^{\numdp - 2} (\dpid = \agent) \Rightarrow (\nextdpid = \agent) \label{enc:stay_home} 
        %\label{enc:e2}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \conjunctionoveragents & \conjunctionoveractionpoints (\dpload = \prevdpload + \pickup - \dropoff) \wedge (\neg(\dpid = \agent) \Rightarrow (\neg(\prevdpid = \dpid))) \label{enc:load_tracking_and_doing_tasks}
        %\label{enc:e3}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \conjunctionoveragents & \bigwedge \nolimits_{\dpvar = \delta_{\agent}}^{\numdp - 1} (\dpid \geq \numagents) \Rightarrow \notag \\
        & (\dptime = ITE(\prevdptime \leq t_j, t_j, \prevdptime) + Dist(Loc(\prevdpid), Loc(\dpid)) + \rho) \label{enc:doing_tasks}
        %\label{enc:e4}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
    %General uninterpreted function restriction:
        \conjunctionoverlocations[\location_1] & \conjunctionoverlocations[\location_2] Dist(\location_1, \location_2) = w_{\location_1, \location_2} \conjunctionoveragents Loc(\agent) = n_s \label{enc:room_UF_agents_and_dist_UF}
        %\label{enc:e5}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
    %Bounding action point values:
        \conjunctionoveragents &
        \conjunctionoveractionpoints (\dpload \geq 0) \wedge (\dpload \leq \capacity) \wedge (\dpid \geq 0) \wedge (\dpid = \agent) \Rightarrow (\dptime = t_{max}) \label{enc:bound_load_bound_id_go_home}
        %\label{enc:e6}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \iffalse
        \conjunctionoveragents & \bigwedge \limits_{\dpvar = 1}^{\numdp - 1} (\dpid = \agent) \Rightarrow (\dptime = t_{max}) \label{enc:go_home} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \conjunctionoveragents & \bigwedge \limits_{\dpvar = 1}^{\numdp - 1} \neg(\dpid = \agent) \Rightarrow (\dpid \geq \numagents) \label{enc:at_home_or_doing_task} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \fi
        \conjunctionoveragents & \bigwedge \limits_{\dpvar = 1}^{\numdp - 1} \neg(\dpid = \agent) \Rightarrow (\validid) \label{enc:at_home_or_doing_task_with_id}
        %\label{enc:e7}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
    %Task uninterpreted function restriction:
        \conjunctionovertasks & (Loc(2\task + \numagents) = m_{s_i}) \wedge (Loc(2\task + \numagents + 1) = m_{s_f}) \label{enc:room_UF_task_rooms} 
        %\label{enc:e8}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
    %Relating action and task tuples:
        \conjunctionoveragents & \conjunctionoveractionpoints \conjunctionovertasks (\dpid = 2\task + \numagents) \Rightarrow ((\taskstarttime = \dptime) \wedge \droplater) \label{enc:started_task} 
        %\label{enc:e9}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \conjunctionoveragents & \conjunctionoveractionpoints \conjunctionovertasks (\dpid = 2\task + 1 + \numagents) \Rightarrow (\taskendtime = \dptime) \wedge (\taskagent = \agent) \label{enc:ended_task} 
        %\label{enc:e10}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
        \conjunctionoveragents & \conjunctionovertasks (\taskagent = \agent) \Rightarrow \agentstarts \label{enc:assigned_agent} 
        %\label{enc:e11}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
        \\
    %Task tuple restriction:
        \conjunctionovertasks & (\taskagent \geq 0) \wedge (\taskagent < \numagents) \wedge (\taskstarttime \geq t_j) \wedge (\taskendtime \leq \taskdeadline)\label{enc:valid_agent_and_times} 
        %\label{enc:e12}
        \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
    \end{align}
    \caption{Constraints used in the encoding developed in Algorithm \ref{alg:overall}}
    \label{fig:encoding}
\end{figure}

\iffalse
\\
\conjunctionovertasks & \taskendtime \geq \taskstarttime + Dist(Loc(2\task + \numagents), Loc(2\task + \numagents + 1)) \label{enc:enough_travel_time} \stepcounter{encodingcounter} \tag{E.\theencodingcounter}
\fi
